Search-based DNN Testing and Retraining with GAN-enhanced Simulations

In safety-critical systems (e.g., autonomous vehicles and robots), Deep Neural Networks (DNNs) are becoming a key component for computer vision tasks, particularly semantic segmentation. Further, since the DNN behavior cannot be assessed through code inspection and analysis, test automation has become an essential activity to gain confidence in the reliability of DNNs. Unfortunately, state-of-the-art automated testing solutions largely rely on simulators, whose fidelity is always imperfect, thus affecting the validity of test results. To address such limitations, we propose to combine meta-heuristic search, used to explore the input space using simulators, with Generative Adversarial Networks (GANs), to transform the data generated by simulators into realistic input images. Such images can be used both to assess the DNN performance and to retrain the DNN more effectively. We applied our approach to a state-of-the-art DNN performing semantic segmentation and demonstrated that it outperforms a state-of-the-art GAN-based testing solution and several baselines. Specifically, it leads to the largest number of diverse images leading to the worst DNN performance. Further, the images generated with our approach, lead to the highest improvement in DNN performance when used for retraining. In conclusion, we suggest to always integrate GAN components when performing search-driven, simulator-based testing.

==> approach_old.tex <==
% !TEX root =  MAIN.tex
\section{The \APPR Approach}
\label{sec:approach}
%In this section, we propose \APPR, a solution based on generative adversarial models and genetic algorithms. The goal of \APPR is to improve DNN performance by identifying and generating synthetic data for rare or dangerous scenarios (i.e. data points that are either infrequent in the real world or pose significant risks. ), as well as those under-represented in real-world training data. Such scenarios are critical to ensure the robustness and safety of DNNs, especially in critical applications, such as autonomous driving and medical diagnosis. 
\APPR supports the testing and improvement of vision DNNs by generating realistic but synthetic inputs belonging to distinct situations. Such realistic inputs are generated by combining meta-heuristic search, simulators, and GANs. Simulators enable the cheap generation of input images and corresponding ground truth information (e.g., correct segmentation mask)
%cheap generation of labeled input images, 
%(compared to manual labelling of real-world images), 
while meta-heuristic search enables the exploration of the input space (i.e., exercise distinct situations). Finally, GANs enable the generation of high-fidelity images from the simulator data, thus maximizing the likelihood that testing results are representative of what observable with real-world inputs, and, in turn, ensuring that the failures observed during testing are due to DNN limitations that can be experienced in the real-world and do not depend on the fidelity gap of simulators. Further, they can be used to retrain the DNN under test to improve its performance with real-world inputs. Last, the images generated by \APPR belong to distinct situations that are unsafe (i.e., the DNN performs poorly), thus enabling the identification of multiple DNN limitations and their improvement. 
%The combined approach of simulators and GANs thus enhances the generalization capability of DNNs by exposing them to a broader range of scenarios and challenges. Simulators offer a controlled environment for generating initial, artificial data on rare or dangerous scenarios, which serves as input for the GANs. The GANs then refine this data, producing synthetic but high-quality and realistic scenarios that the genetic algorithms evaluate and select based on the targeted fitness criteria. 


Figure \ref{fig:approach} provides an overview of \APPR, which consists of three components: 
\begin{enumerate}
\item GAN-based input generation component. It receives as input the configuration parameter values to be used to generate, with a simulator, \emph{scene data} (i.e., an image and the corresponding segmentation map). The scene data is then used to generate a realistic image with a GAN trained on a specific reference domain. In our empirical assessment, we use the Pix2PixHD GAN trained on the CityScape dataset to generate realistic road scenes from the segmentation map produced by the simulator.
%simulates road scenarios and generates a realistic scenario from simulated ones.

\item Fitness computation component. Since we aim to identify situations that are both unsafe (i.e., leading to inaccurate DNN prediction) and different we apply two distinct fitness functions: $F_{accuracy}$, which measures how accurate is the DNN prediction on the generated realistic image (e.g., the accuracy of the semantic segmentation), and $F_{similarity}$, which measures how similar a generated image is from the already generated ones.  These functions enable relying on a minimization algorithm to address our objectives.
%others For each generated realistic image, we compute two fitness values: the quality of an individual () and how diverse it is from the already selected scenarios ().

\item Search Algorithm. We rely a many-objective search algorithm to find a population of diverse situations where the DNN fares poorly, thereby suggesting these scenarios are not well captured by the real-world dataset. In our search algorithm, an individual is captured by the set of parameters used to deterministically generate, using a simulator, scene data, and to derive a realistic image from such a scene data. For optimization purposes, for each individual, we store the simulator parameter values, the scene data, and the realistic image.

\end{enumerate}

The output of \APPR is a set of diverse realistic images leading to poor DNN performance. They should be inspected for safety-analysis purposes; specifically, they enable understanding the situations in which the DNN may fail, determine their likelihood based on domain knowledge, and identify countermeasures. Also, they can be used to retrain the DNN and improve the DNN performance. The following sections provide details about our components.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/GAN-Test2.pdf}
    \caption{Overview of \APPR.}
    \label{fig:approach}
\end{figure*}


%The steps of our approach are described in the following:
\subsection{GAN-based input generation}
\label{sec:approach:inputGeneration}
We generate scene data (i.e., simulated images and corresponding segmentation masks) by relying on the AirSim simulator (Section \ref{sec:airsim}); however, our approach can be applied with simulators having similar capabilities (e.g., Carla~\cite{carla} and BeamNG~\cite{beamng}). To assess DNNs that control a vehicle (e.g., segmentation of the images in front of the vehicle, or steering angle prediction) it is necessary to generate scenes that mimic what observable by a car on the road. Consequently, we control the generation of scene data through two parameters: orientation and position of the car.
 To test other DNNs (e.g., visual navigation for drones), a different set of parameters might be considered (e.g., altitude might be included).


% \subsubsection{Image Simulator - AirSim}
% \label{sec:simulator}
% To simulate scenarios not well-captured by the real-world dataset, we employ the AirSim simulator (Section \ref{sec:airsim}). This platform provides a realistic and customizable environment for generating diverse scenarios, including challenging lighting conditions, terrain variations, and object placements. We utilize AirSim to simulate rare scenarios, capturing situations that may not be available in real-world datasets. Utilizing a simulator also allows for the creation of different driving situations by adjusting the simulator's controllable parameters, e.g., orientation and position of the car in our study. Scenarios generated by Airsim are represented as simulated images and segmentation masks they are associated with (ground truth). 

We generate realistic images from the ground truth information provided by the simulator. In our experiments, such ground truth is the segmentation mask, but could be different information in other contexts.
To this end, we utilize a Pix2PixHD DNN~\cite{wang2018pix2pixHD} that we train using the same dataset used for the DNN under test; such dataset consists of pairs $\langle \text{image}, \text{expected output} \rangle$. For example, in our experiments, we considered a DNN trained on a dataset of pairs $\langle \text{European road image}, \text{segmentation mask} \rangle$, which we use to train Pix2PixHD to generate images of roads belonging to European cities from segmentation masks.

To generate realistic images during testing, \APPR provides the ground truth of the simulated image to the trained Pix2PixHD to generate a realistic image; in our experiments, \APPR provides to Pix2PixHD the segmentation mask produced by AirSim in order to generate realistic images resembling real-world images from Cityscapes.


% \subsubsection{Data Preprocessing}

% In semantic segmentation tasks, each distinct object in a scene is denoted by a specific color. This color assignment serves as a 'label' for the object, facilitating its identification and differentiation from other elements within the image. However, a significant challenge arises due to the discrepancy in color coding (label assignment) between the objects as represented in the source and target datasets (e.g., segmentation provided by the simulator and the one from the dataset used to train the DNN). 

% The process of data preprocessing involves relabelling the segmentation masks to ensure compatibility between the different labels. This process involves creating a new mapping scheme where each label from the source dataset (identified by its unique color in the segmentation masks) is reassigned to match the corresponding label (and its color code) in the target dataset.

% The mapping between Cityscapes labels and Airsim labels is presented in Table \ref{tab:mapping}.
% \input{tables/mapping}





\subsection{Fitness Functions}


\subsubsection{Accuracy fitness}

The fitness function $F_{accuracy}(i)$, which computes the accuracy of the DNN on an individual, depends on the DNN under test. In general, we suggest relying on the metric used to measure the performance of the DNN. For example, in our empirical assessment, we test a DNN for image segmentation whose performance is measured with the \emph{mean Intersection over Union (mIoU)} metric, also known as Jaccard Index~\cite{everingham2010pascal}. It measures the overlap between the predicted segmentation mask and the ground truth mask for a class (e.g., car, road, ect.). The IoU value is calculated as the ratio of the intersection area to the union area of the two masks. The mean IoU for one image is obtained by averaging the IoU scores across all classes.
%IoU provides a comprehensive evaluation by measuring the overlap between the predicted bounding boxes or segmentation masks and the ground truth annotations of vehicles in images or point clouds. In autonomous driving, where precise identification and localization of cars are crucial for safe navigation, IoU serves as a reliable metric to quantify the performance of detection and segmentation algorithms.
 However, in our case study, we focus on a specific capability of the DNN, which is its ability to detect cars accurately; our choice is due to cars being the most significant object on the road. 
 %is crucial for safety in autonomous driving, we only focused on the car object when computing the fitness. Prioritizing IoU for cars ensures robust detection and tracking performance specifically tailored to the most significant objects on the road.
 Therefore, we compute $F_{accuracy}(i)$ by relying on the IoU formula for car objects:
 
\begin{equation}
IoU_{car}(i) = \frac{{TP_{car}(i)}}{{TP_{car}(i) + FP_{car}(i) + FN_{car}(i)}}
\end{equation}

where $TP_{car}(i)$ are the true positive car pixels in image $i$ (pixels that belong to cars in both ground truth and prediction), $FP_{car}(i)$ are the false positive pixels for cars (pixels erroneously reported as belonging to a car in the predicted segmentation mask), and $FN_{car}(i)$ are the false negative pixels (pixels erroneously not reported as belonging to a car in the predicted segmentation mask).

Unfortunately, when test images are automatically generated using simulators and GANs, the DNN may badly perform because the generated images are non-relevant for testing, specifically, they may be out-of-distribution (because of simulator's limitations) or may not match the ground truth (because of GAN's limitations). 
Consequently, we defined a fitness function that distinguishes between non-relevant and relevant individuals, as follows:
%performance metrics are not sufficient to capture the quality of an individual. Indeed, both simulators and GAN may lead to non-relevant images. It is therefore necessary to define a fitness function that first verifies if the image is not relevant and then compute the performance metric, as follows:

\begin{equation}
F_{accuracy} (i) =  
    \begin{cases}
      2 & \text{if } i \text{ is not relevant}\\
      \mathit{performance}(i) & \text{otherwise}
    \end{cases}   
\end{equation}

We assume the performance metric (i.e., $performance(i)$) to be normalized in the range 0-1, with a perfect output leading to $1$. Therefore, since in our search we aim to minimize the fitness function, we return a fitness of 2 for non-relevant individuals, so that they are discarded by the search process. 

Determining the degree of realism of an input depends on the specific case study.
In our empirical study, for example, we observe out-of-distribution inputs when the ego vehicle is positioned next to another vehicle and perpendicular to it (e.g., facing the other vehicle's door), which is not interesting for our testing purposes because it is very easy to make a segmentation DNN fail in such case.
%, and therefore we aim to ignore them. 
Another case is that of images with no cars, which should be excluded because we are interested in testing the DNN with images with traffic. Consequently, we consider an image to be relevant if the proportion of pixels  belonging to cars (i.e., $\mathit{carPixelsProportion}$) in the input image are within a given range:
$$0<\mathit{carPixelsProportion}<40$$ 
%$T_{pp_{high}}$
%introduced a threshold $T_{proportion}$ for the proportion of the car pixels in the input to 
We set the upper bound to $40$ to ensure that the car does not cover most of the image. 
%This threshold helps maintain realistic scenes by preventing the car from dominating the image, thereby allowing for a more diverse and representative dataset. 
%By setting a threshold, it ensures that 
%and other elements such as road, buildings, pedestrians, and signs are appropriately represented in the simulated environment. 
We set the lower bound above zero to ensure that the image contains at least one car. The \emph{carPixelsProportion} is  computed on the segmentation ground truth.
%thus enhancing the diversity and the realism of the training data for the autonomous driving system. 
%$T_{proportion}$ is equal to 40\% of the image to make sure the car doesn't cover the view, and 0\% to ensure the presence of a car in the image.

%The presence of a simulator is not the only reason for lack of realism. Indeed, GAN outputs may not accurately capture what is depicted in the simulator output. For example, we cannot be sure if in our case study the GAN correctly generates car shapes. 
Unfortunately, only humans can determine if a GAN-generated realistic image is a correct representation of the ground truth (i.e., cars really appear where car pixels are reported on the ground truth).
%the realism of an image can only be done by a human, which is not feasible when GAN-based image generation is triggered by a genetic algorithm. 
%Therefore, since we rely on a generative model to generate realistic images from simulated ones, some images might lack realism, e.g., a car can be present in a simulated image but not in the realistic image. However, it is infeasible to check the realism of an image visually. 
However, to automate such verification, we propose relying on heuristics based on the difference in DNN performance observed with images generated by the simulator and images generated by corresponding realistic images. 
Our heuristic relies on the empirical observation that the DNN under test performs better on a realistic image than on the corresponding simulator image, which is expected with DNNs trained on real-world images, not simulator images. 
%performance observed with images simulated and realistic images, we introduced an automated technique to assess the realism of images. 
To apply our heuristic, before testing, we consider a large set  of simulator images  generated with randomly selected parameter values, and generate corresponding realistic images. For example, we generated 1000 images in our empirical assessment. Each simulator and realistic image is processed by the DNN under test to generate a prediction, and the performance metric is computed for each, which enables computing the performance difference as: 
$$\mathit{delta}_{performance}(i) = \mathit{performance}_{simulated}(i) - \mathit{performance}_{realistic}(i)$$
with $i$ indicating the i-th pair of simulator and corresponding realistic image.

After sorting the generated image pairs based on their $\text{delta}_{performance}(i)$, it is possible, through visual inspection, to determine a threshold ($T_{relevance}$) above which the realistic images do not correctly capture the ground truth (e.g., a car is missing where expected, in our case study subject).
During testing, we thus consider a realistic image to be relevant if ${delta}_{performance}(i)<T_{relevance}$. For the segmentation DNN considered in our empirical assessment:
$$\mathit{delta}_{performance}(i) = \mathit{delta}_{IoU}(i) = \mathit{IoU}_{simulated}(i) - \mathit{IoU}_{realistic}(i)$$,
and we selected $T_{relevance}$ as the third percentile of $\mathit{delta}_{performance}$ distribution.

%We assume that a DNN will perform better on a realistic image than on a simulated one because it is pre-trained on Cityscapes, a dataset of real world images. Given this assumption, we define as non-relevant images all the scenarios where the DNN performs better on the corresponding simulated image than on the realistic one. To automatically find non-relevant scenarios, we use the DNN to generate a prediction from the simulated image, we compute the $IoU_{car}$ denoted as $IoU_{simulated}$. We then compute $delta_{IoU} = IoU_{simulated}$ - $IoU_{realistic}$. We set a realism threshold, called $T_{realism}$, as the third quartile of the $delta_{IoU}$ distribution computed on a set of 1000 randomly generated scenarios, which is equal to $0.1$. A scenario is considered relevant if its  $delta_{IoU} < T_{realism}$. 


%$F_{quality}$ is then measured based on the $IoU_{car}$ of the new individual, $T_{proportion}$, and $T_{realism}$ as explained in Equation \ref{eq:f1}. 

Finally, to prevent the positioning of the car outside of the road (e.g., on a building), we ensure that the position of the car is within the road lanes, whose coordinates we mapped manually, otherwise a high fitness is returned.

In the segmentation DNN considered in our empirical assessment, $F_{accuracy}$ is therefore computed as follows:
\begin{equation}
\label{eq:f1}
F_{accuracy} (i) =  
    \begin{cases}
      2 & \text{if } {delta_{IoU}(i) > T_{relevance}}\\
      2 & \text{if } {0}<\mathit{pixelsProportion}<{40}\\
      2 & \text{if } \text{the ego vehicle is outside the road}\\
      %1 & \text{if archive is empty}\\ archive is never empty
      IoU_{car}(i) & \text{otherwise}
    \end{cases}   
\end{equation}

% \begin{algorithm}[H]
% \caption{$F_{quality}$ computation}
% \label{alg:f1}
% \begin{algorithmic}[1]
% \Require $delta_{IoU}$, ${proportion_{car}}$
% \Ensure $F_{quality}$
% \If{$delta_{IoU} > T_{realism}$ or $0\% \geq proportion_{car} \geq 40\%$}
%     \State $F_{quality} \gets \infty$
% \Else
%     \State $F_{quality} \gets IoU_{car}$
% \EndIf
% \end{algorithmic}
% \end{algorithm}

\subsubsection{Diversity fitness}

Our diversity fitness should enable determining if a newly generated image captures a situation not observed before (e.g., no traffic on the road VS a lot of traffic on the road), which could be achieved by computing the difference between the newly generated image and the previously generated images (e.g., stored in an archive). However, the above-mentioned objective it's unlikely achievable with a simple computation of the distance as difference between two matrices, each having the RGB pixel values of one image; indeed, two images generated before and after slightly turning a car, may present pixels that are all shifted in one direction thus resulting into a high difference even if the two images capture the same situation. 

To address the problem above, we suggest capturing the semantic difference between two images by computing the difference between the feature vectors derived from the two images.
Specifically, based on our previous experience with clustering of DNN failures~\cite{Mohammed:PipelinesAssessment}, we rely on a ResNet50 model trained on the ImageNet dataset to automatically derive feature vectors. The deep architecture of ResNet50 (50 layers) allows it to capture richer and more abstract features at different levels of the network. This makes it more powerful for feature extraction tasks where high-level semantic features are important~\cite{he2016deep, simonyan2015very}. Feature vectors should capture the high-level characteristics present in the image; by relying on ResNet50 to identify such feature vectors, we assume, supported by our previous work, that such DNN can automatically encode the relevant information characterizing an image.
Image diversity can be then computed as the Euclidean distance between two feature vectors.
%as the feature-based Euclidean distance from the nearest image in an archive ($\mathit{distanceFromClosest}$). 
Euclidean distance inherently measures the geometric distance between points in a multi-dimensional space. When applied to feature vectors representing images, it captures the differences in features between images. Images with similar features will have a shorter distance, indicating less diversity, while images with dissimilar features will have a longer distance, suggesting higher diversity. 
%The features are extracted using a ResNet50 model pre-trained on ImageNet dataset.

In the presence of an archive with previously generated images, $F_{similarity}$, which should capture how $i$ is similar to previously generated images, can thus be computed as an inversely proportional function of the Euclidean distance from the closest image in the archive. However, in a search algorithm, preserving images that slightly differ from previously generated ones may lead to being stuck in local optima; therefore, inspired by previous work \cite{riccio2020model}, we introduce a threshold for the diversity ($T_{diversity}$) below which an image is not considered different from a previously generated one and is thus assigned with high fitness:


\begin{equation}
\label{eq:f2}
F_{similarity} (i) =  
    \begin{cases}
      2 & \text{if } \mathit{distanceFromClosest}
    (i) < T_{diversity}\\
      %1 & \text{if archive is empty}\\ archive is never empty
      1 / (1 + \mathit{distanceFromClosest}_
    (i)) & \text{otherwise}
    \end{cases}   
\end{equation}

The value of $\mathit{distanceFromClosest}_(i)$ is identified by computing the Euclidean distance of the image $i$ from each image in the archive and selecting the shortest one. 
%We also introduce a threshold for the diversity $T_{diversity}$ inspired from the work of Riccio et al. \cite{riccio2020model}. 
Like in related work~\cite{riccio2020model}, we compute $T_{diversity}$ as the median of the pairwise distances in a set of 1000 randomly generated images. %It is equal to 14 in our study. 
Finally, the term $1 / (1 + \mathit{distanceFromClosest}_(i))$ is used as a normalization factor for an unbound distance; it leads to a fitness close to zero for a very high distance, and to one for overlapping images.



% \begin{algorithm}
% \caption{$F_{diversity}$ computation}
% \label{alg:f2}
% \begin{algorithmic}[1]
% \Require \text{distance\_closest}, $T_{diversity}$
% \Ensure  $F_{diversity}$
% \If{$\text{distance\_closest} > T_{diversity}$}
%    \State $F_{diversity} \gets \text{distance\_closest}$
%    \State Add image to archive
% \ElsIf{$\text{distance\_closest} < T_{diversity}$ \textbf{and} $F1_{closest} > F1_{new}$}
%   \State Replace closest image with new image in the archive
% \Else
%    \State $F_{diversity} \gets \infty$
% \EndIf
% \end{algorithmic}
% \end{algorithm}



%where \text{distance\_closest} is the distance to the nearest image in the archive.


\subsection{Search algorithm}
\label{sec:genetic}
We aim to address a multi-objective problem, trying to generate realistic images leading to minimal DNN accuracy and having minimal similarity among each other. We therefore rely on the NSGA-II algorithm, which demonstrated its effectiveness in multiple multi-objective software testing problems. However, inspired by related work aiming at maximizing the diversity among the generated individuals~\cite{riccio2020model}, 
%minimize the accuracy ofTo identify scenarios not adequately captured by the real-world dataset on which the DNN was trained, we employ a search algorithm with two objectives: the quality and the diversity of an individual (scenario). The problem addressed in our paper is similar to the one addressed by related works like DeepJanus \cite{riccio2020model}. Therefore, inspired by the latter, 
we extend NSGA-II with an archive to store the best (non-dominated) individuals encountered during the search process. The archive plays a critical role in preventing the genetic algorithm from cycling, a phenomenon where the population moves from one area of the solution space to another and then back again without exploring other areas.
%any memory of the areas it has already explored. 
By retaining the best individuals in the archive, and assigning high fitness values to individuals that are similar to the already generated ones, the algorithm ensures that these areas are not revisited unnecessarily, facilitating a more efficient exploration of the solution space. 



%For every newly generated image, we calculate its distance to the nearest image in the archive. If the distance falls below $T_{diversity}$, we include the new image in the archive. However, if the distance is below $T_{diversity}$, indicating a lack of diversity, it may yet hold potential for enhancing $F_{quality}$, and so we compare $F1_{new}$ with $F1_{closest}$. If $F1_{new}$ is lower than $F1_{closest}$, we substitute the closest image in the archive with the new one. $F_{diversity}$ is computed based on $T_{diversity}$ as explained in Equation \ref{eq:f2}.

\begin{algorithm}[t]
\caption{Updating the archive with image i}
\label{alg:update}
\begin{algorithmic}[1]
\Require $A$: archive with individuals selected so far, $i$: individual to be added, $T_{similarity}$
\Ensure  archive with individuals that are sparse and minimize $F_{accuracy}$
\If{$F_{accuracy}(i) == 2$} \Comment{ignore unrealistic individuals}\label{algo:archive:ignore:unrealistic}
   \State return 
\EndIf   
\If{$\mathit{distanceFromClosest}(i) > T_{diversity}$} \Comment{add diverse and realistic individuals}
   \State add i to $A$ \label{algo:archive:include:distant}
\ElsIf{$\mathit{distanceFromClosest}(i) \leq T_{diversity}$ \textbf{and} $F_{quality}(closestTo(i)) > F_{quality}(i)$}
  \State put $i$ in the archive $A$ in place of its closest individual already in the archive \label{algo:archive:include:lowerAcc}
\EndIf
\end{algorithmic}
\end{algorithm}

Before describing our search algorithm, we describe the procedure adopted to update the archive with an individual $i$, which is shown in Algorithm~\ref{alg:update}. 
Individuals that are non-relevant for testing (i.e., $F_{accuracy}(i) == 2$) are not added to the archive (Line~\ref{algo:archive:ignore:unrealistic}). Instead, we add individuals that are relevant and dist from the closest individual in the archive more than the predefined threshold (Line~\ref{algo:archive:include:distant}).
Last, since individuals that are similar to others in the archive (i.e., $\mathit{distanceFromClosest}(i) < T_{diversity}$) may still be more effective for testing (i.e., lower $F_{accuracy}$) we put the individual $i$ in place of the individual that is closest to $i$ in the archive, when the $F_{accuracy}$ of the former is lower than the accuracy of the latter (Line~\ref{algo:archive:include:lowerAcc}).
%, with $closestTo(i)$ being the individual already in the archive that is closest to $i$).

% The genetic algorithm operates on the semantic segmentation outputs of the DNN. It evaluates different simulated scenarios by calculating each scenario's $F_{quality}$ and $F_{diversity}$. $F_{quality}$ is used to assess the quality of a simulated scenario. The images that result in lower $F_{quality}$ values are critical as they highlight scenarios where the DNN's interpretation of the data is less accurate, signaling areas where the model's understanding of the semantic segmentation needs improvement. $F_{diversity}$ aims at maximizing the diversity of the simulated scenarios generated by AirSim. The $F_{diversity}$ metric quantifies the diversity and variety of test scenarios within which the DNN's performance is assessed. A higher $F_{diversity}$ denotes a more varied set of conditions, ensuring an exhaustive assessment of the DNN's robustness and versatility. Focusing on diversity ensures the model confronts an extensive range of real-world situations, exposing subtle or rare complexities not present in the initial training dataset.





\begin{algorithm}[t]
\caption{Search algorithm used in \APPR}
\label{alg:search}
\begin{algorithmic}[1]


\Require $g_{max}$: maximum number of generations, $N$: population size, $P_c$: crossover probability, $P_m$: mutation probability, $r$: number of populations for initial seed selection
\Ensure An archive of best individuals 
\State Initialize an empty archive $A$ (a set of individuals) \label{algo:search:createArchive}
\State Initialize $r$ random populations $P^0_0$..$P^r_0$ with $N$ simulated scenarios in each population \label{algo:search:start}
\State Evaluate $F_{accuracy}$ and $F_{similarity}$ of each individual in each population $P_0$ based on Equation \ref{eq:f1} and Equation \ref{eq:f2}
\State Select the population $P_0$ that includes the individual with the lowest $F_{accuracy}$. \label{algo:search:select:start}
\State Update the archive $A$ based on $F_{quality}$ and $F_{diversity}$ of each individual in $P_0$ \label{algo:search:firstUpdate}
\State Rank the population using non-dominated sorting \label{algo:search:sort}
\State Calculate crowding distance for each individual \label{algo:search:crowd}
\State $g \gets 1$
\While{$g < g_{max}$}
    \State Select parents from current population $P_g$ using binary tournament selection based on rank and crowding distance \label{algo:search:parents}
    \State Generate offspring $Q_g$ using polynomial mutation and simulated binary crossover \label{algo:search:offspring}
    \State Combine $P_g$ and $Q_g$ into $R_g$
    \State Compute $F_{accuracy}$ and $\mathit{distanceFromClosest}$ of each individual in $R_g$ \label{algo:search:compute:metrics}
    \State Update the archive $A$ based on Algorithm~\ref{alg:update}  \label{algo:search:loop:update}
    \State Evaluate $F_{similarity}$ of each individual $R_g$ \label{algo:search:loop:diversity}
    \State Rank $R_g$ using non-dominated sorting \label{algo:search:loop:rank}
    \State Calculate crowding distance for each individual in $R_g$ \label{algo:search:loop:crowd}
    \State Select the top $N$ individuals from $R_g$ to form new population $P_{t+1}$ based on rank and crowding distance \label{algo:search:loop:select}
    % \State $t \gets t + 1$
    \State $g \gets g + 1$
    
\EndWhile
%\State \textbf{return} the first front of $P_g$ as the set of non-dominated solutions
\State \textbf{return} the archive $A$

\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:search} presents the pseudocode of the NSGA-II algorithm with archive employed in \APPR. After creating an empty archive (Line~\ref{algo:search:createArchive}),
since the initial selection of seeds may affect the search results, inspired by our previous work~\cite{SAFE}, we generate multiple ($5$ in our experiments) populations of $N$ randomly selected individuals (Line~\ref{algo:search:start}) and we select the population with the individual having the lowest $F_{accuracy}$ (Line~\ref{algo:search:select:start}). All the individuals in $P_0$ are then used to update the archive based on Algorithm~\ref{alg:update} (Line~\ref{algo:search:firstUpdate}). Shortly, the archive is populated with the individuals that dist more than $T_{diversity}$ and lead to worst accuracy.

As per NSGA-II, the population undergoes a non-dominated sorting process and crowding distance calculation (Lines \ref{algo:search:sort}-\ref{algo:search:crowd}).

The algorithm's core is a loop that iterates until the generation count reaches the specified maximum $g_{max}$. Within each generation $g$, we use NSGA-II's tournament selection method to select parent individuals for the next generation (Line~\ref{algo:search:parents}). 
%During the tournament, individuals are first compared based on their non-domination levels (rankings), with those having lower ranks (indicating superior multi-objective performance) being preferred. Suppose two individuals have the same rank; the one with a higher crowding distance (indicating a larger surrounding empty space in the objective space, hence contributing more to diversity) is selected. This process ensures a balanced population advancement towards the Pareto front, maintaining diversity while optimizing both objectives simultaneously.
Offspring generation follows, employing polynomial mutation and simulated binary crossover (Line~\ref{algo:search:offspring}).
%crossover and mutation techniques (line 11). To generate offspring $Q_g$, selected parents undergo crossover and mutation operations. Crossover combines the traits of two parents to produce new offspring, while mutation introduces random changes to an individual's traits. These operations are crucial for introducing genetic diversity and exploring new areas of the input space that may reveal additional weaknesses in the DNN. Our approach uses NSGA's polynomial mutation and simulated binary crossover.
Then, we compute $F_{quality}$ and $\mathit{distanceFromClosest}$ for each individual in $R_g$ (Line~\ref{algo:search:compute:metrics}, with $R_g$ being the union of the current population $P_g$ with the offspring population $Q_g$). 
Recomputing $\mathit{distanceFromClosest}$ for the individuals in the parent population is necessary because, in the previous iteration, new individuals had been added to the archive and, therefore, distances changed. 
%The current population $P_g$ is merged with the offspring population $Q_g$ to form $R_g$ (line 12). Then, each individual's $F_{quality}$ and $\mathit{distanceFromClosest}$ are computed (line 13). 
The archive is then updated based on Algorithm \ref{alg:update} (Line \ref{algo:search:loop:update}), and each individual's $F_{diversity}$ is computed (Line~\ref{algo:search:loop:diversity}). 
$R_g$ is then ranked using the non-dominated sorting process (Line \ref{algo:search:loop:rank}) and the top individuals, based on rank and crowding distance, form the new population $P_{t+1}$ for the subsequent generation (Lines \ref{algo:search:loop:crowd}-\ref{algo:search:loop:select}).

The algorithm concludes by returning an archive of non-dominated solutions as the optimal outcome of the search process.


==> tables/mapping.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Object} & \textbf{Cityscapes RGB Color} & \textbf{Airsim RGB Color} \\ \hline
Road & [128, 64, 128] & [142,1,246] \\ \hline
Sidewalk & [244, 35, 232] & [112,105,191] \\ \hline
Building & [70, 70, 70] & [59,37,212] \\ \hline
Wall & [102, 102, 156] & [203,102,204] \\ \hline
Fence & [190, 153, 153] & [115,176,195] \\ \hline
Pole & [153, 153, 153] & [109,206,24] \\ \hline
Traffic Light & [250, 170, 30] & [240,59,210] \\ \hline
Traffic Sign & [220, 220, 0] & [32,151,196] \\ \hline
Vegetation & [107, 142, 35] & [232,250,80] \\ \hline
Terrain & [152, 251, 152] & [128, 128, 0] \\ \hline
Sky & [70, 130, 180] & [0, 0, 0] \\ \hline
Person & [220, 20, 60] & [189,135,188] \\ \hline
Rider & [255, 0, 0] & [128, 0, 128] \\ \hline
Car & [0, 0, 142] & [184,145,182] \\ \hline
Truck & [0, 0, 70] & [128, 128, 128] \\ \hline
Bus & [0, 60, 100] & [0, 128, 255] \\ \hline
Train & [0, 80, 100] & [128, 0, 255] \\ \hline
Motorcycle & [0, 0, 230] & [255, 128, 128] \\ \hline
Bicycle & [119, 11, 32] & [119,180,120] \\ \hline
\end{tabular}
\caption{Mapping of the labels between Cityscapes and Airsim}
\label{tab:mapping}
\end{table}
